SemRel2024: A Collection of Semantic Textual Relatedness Datasets for 13 Languages

Exploring and quantifying semantic relatedness is central to representing language and holds significant implications across various NLP tasks. While earlier NLP research primarily focused on semantic similarity, often within the English language context, we instead investigate the broader phenomenon of semantic relatedness. In this paper, we present \textit{SemRel}, a new semantic relatedness dataset collection annotated by native speakers across 13 languages: \textit{Afrikaans, Algerian Arabic, Amharic, English, Hausa, Hindi, Indonesian, Kinyarwanda, Marathi, Moroccan Arabic, Modern Standard Arabic, Spanish,} and \textit{Telugu}. These languages originate from five distinct language families and are predominantly spoken in Africa and Asia -- regions characterised by a relatively limited availability of NLP resources. Each instance in the SemRel datasets is a sentence pair associated with a score that represents the degree of semantic textual relatedness between the two sentences. The scores are obtained using a comparative annotation framework. We describe the data collection and annotation processes, challenges when building the datasets, baseline experiments, and their impact and utility in NLP.

==> tables/bert_baselines.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\tiny
\begin{tabular}{@{}lllllllllllll@{}}
\toprule
\textbf{Language} &
  \textbf{MARBERT} &
  \textbf{afro-xlmr-large} &
  \textbf{albert-base-spanish} &
  \textbf{am-roberta} &
  \textbf{bert-base-arabert} &
  \textbf{bert-base-arabic} &
  \textbf{mBERT} &
  \textbf{bert-base-spanish-wwm-cased} &
  \textbf{dziriBERT} &
  \textbf{IndicBERT} &
  \textbf{roberta-base-bne} &
  \textbf{XLMR} \\ \midrule
afr & -    & 0.45 & -    & -    & -   & -    & 0.74  & -    & -    & -     & -    & 0.56  \\
amh & -    & 0.4  & -    & 0.72 & -   & -    & 0.13  & -    & -    & -     & -    & 0.57  \\
arb & 0.29 & 0.18 & -    & -    & 0.3 & 0.31 & 0.42  & -    & -    & -     & -    & 0.32  \\
arq & -    & -    & -    & -    & -   & -    & 0.37  & -    & 0.43 & -     & -    & 0.25  \\
ary & -    & -    & -    & -    & -   & -    & 0.27  & -    & -    & -     & -    & 0.17  \\
eng & -    & 0.3  & -    & -    & -   & -    & 0.68  & -    & -    & 0.61  & -    & 0.6   \\
esp & -    & -    & 0.62 & -    & -   & -    & 0.66  & 0.68 & -    & -     & 0.66 & 0.69  \\
hau & -    & 0.07 & -    & -    & -   & -    & 0.16  & -    & -    & -     & -    & 0.04  \\
hin & -    & -    & -    & -    & -   & -    & 0.62  & -    & -    & 0.4   & -    & 0.51  \\
ind & -    & -    & -    & -    & -   & -    & 0.5   & -    & -    & -     & -    & 0.47  \\
kin & -    & 0.16 & -    & -    & -   & -    & 0.12  & -    & -    & -     & -    & 0.13  \\
mar & -    & -    & -    & -    & -   & -    & 0.65  & -    & -    & 0.46  & -    & 0.6   \\
pan & -    & -    & -    & -    & -   & -    & -0.16 & -    & -    & -0.16 & -    & -0.07 \\
tel & -    & -    & -    & -    & -   & -    & 0.66  & -    & -    & 0.41  & -    & 0.58  \\ \bottomrule
\end{tabular}
\caption{Spearman correlation scores for BERT-based models with cosine similarity and without further fine-tuning.}
\label{tab:encoder-based-models}
\end{table*}

==> tables/language_specific_bert.tex <==

\begin{table}[]
\tiny
\begin{tabular}{@{}cc@{}}
\toprule
\textbf{Language} & \textbf{\begin{tabular}[c]{@{}c@{}}Language-Specific\\  BERT\end{tabular}} \\ \midrule
\textbf{afr} & afro-xlmr-large \\
\textbf{amh}      & afro-xlmr-large / am-roberta                                               \\
\textbf{arb}      & MARBERT / afro-xlmr-large / bert-base-arabert / bert-base-arabic           \\
\textbf{arq} & dziribert       \\
\textbf{ary} & -               \\
\textbf{eng} & afro-xlmr-large / bert-base-uncased \\
\textbf{esp}      & albert-base-spanish / bert-base-spanish-wwm-cased / roberta-base-bne       \\
\textbf{hau} & afro-xlmr-large \\
\textbf{hin} & indic-bert      \\
\textbf{ind} & -               \\
\textbf{kin} & afro-xlmr-large \\
\textbf{mar} & indic-bert      \\
%\textbf{pan} & indic-bert      \\
\textbf{tel} & indic-bert      \\ \bottomrule
\end{tabular}
\caption{The above table describes the corresponding language-specific BERT used for the baselines. Refer to the Table \ref{tab:encoder-based-models} for the corresponding scores in the same column.}
\label{tab:language-specific BERT}
\end{table}

==> tables/updated_table.tex <==


% \begin{table*}[]
%     \centering
%     \small
%     \begin{tabular}{ccccccccccccccc}
%         \toprule[1.2pt]
%         \textbf{Model Type} & \multicolumn{14}{c}{\textbf{Languages}} \\
%         \cmidrule(lr){2-15}
%         \midrule
%        \textbf{Language Agnostic} & \multicolumn{14}{c}{} \\
%         \cmidrule(lr){2-15}
%         mBERT & 0.74 & 0.13 & 0.42 & 0.37 & 0.27 & 0.68 & 0.66 & 0.16 & 0.62 & 0.50 & 0.12 & 0.65 & -0.16 & 0.66 \\
%         XLMR & 0.56 & 0.57 & 0.32 & 0.25 & 0.17 & 0.60 & 0.69 & 0.04 & 0.51 & 0.47 & 0.13 & 0.60 & -0.07 & 0.58 \\
%         \midrule
       
%         \textbf{Language Specific} & \multicolumn{14}{c}{} \\
%         \cmidrule(lr){2-15}
%         AfroXLMR & 0.45 & 0.40 & 0.18 & 0.64 & 0.77 & 0.80 & 0.70 & 0.74 & 0.93 & 0.68 & 0.74 & 0.92 & 0.65 & 0.79 \\
%         Indic-BERT & & & & & & & & & & & & & & \\
%         albert-base-spanish & - & - & - & - & - & - & 0.30 & - & - & - & - & - & - & - \\
%         MARBERT & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         ARBERT & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         dziriBERT & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         RoBERTa & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%         \bottomrule[1.2pt]
%     \end{tabular}
%     \caption{Baseline Spearman Correlation Scores for Language-Agnostic and Language-Specific BERT-Based Models Using Cosine Similarity. These are out-of-the-box correlation scores without any fine-tuning
%      % Monolingual BERT models for the corresponding language can be referred to in the following Table \ref{tab:language-specific BERT}. The scores in the Language-specific BERT correspond to the corresponding BERT model in the table
%     .}
%     \label{tab:encoder-based-models}
% \end{table*}

\begin{table*}[!ht]
    \centering
  \small
  %\resizebox{\textwidth}{!}{
%     \begin{tabular}{ccccccccccccccc}
     \begin{tabular}{lcccccccccccccc}
        \toprule[1.2pt]
         %& \multicolumn{14}{c}{\textbf{Languages}} \\
        %\cmidrule(lr){2-15}
         & \texttt{afr} & \texttt{amh} & \texttt{arb} & \texttt{arq} & \texttt{ary} & \texttt{eng} & \texttt{esp} & \texttt{hau} & \texttt{hin} & \texttt{ind} & \texttt{kin} & \texttt{mar} & \texttt{pan} & \texttt{tel}  \\
        \midrule
               %\textbf{Model Type} & \multicolumn{14}{c}{\textbf{Lexical Overlap}} \\
        %\cmidrule(lr){2-15}
        \textbf{Overlap}&0.71 & 0.63 & 0.32 & 0.40 & 0.63 & 0.67 & 0.67 & 0.31 & 0.53 & 0.55 & 0.33 & 0.62 & -0.27 & 0.70 \\        % \cmidrule(lr){2-15}

       %\textbf{} & \multicolumn{14}{c}{\textbf{Unsupervised}} \\
        \midrule
        & \multicolumn{14}{c}{\textbf{Unsupervised (Multilingual)}} \\\cmidrule(lr){2-15}
        \textbf{mBERT} & 0.74 & 0.13 & 0.42 & 0.37 & 0.27 & 0.68 & 0.66 & 0.16 & 0.62 & 0.50 & 0.12 & 0.65 & -0.16 & 0.66 \\
        \textbf{XLMR} & 0.56 & 0.57 & 0.32 & 0.25 & 0.17 & 0.60 & 0.69 & 0.04 & 0.51 & 0.47 & 0.13 & 0.60 & -0.07 & 0.58 \\
        \midrule
        & \multicolumn{14}{c}{\textbf{Unsupervised (Monolingual)}} \\
        \cmidrule(lr){2-15}
        \textbf{AfroXLMR} & 0.45 & 0.40 & 0.18 & - & - & 0.30 & - & 0.07 & - & - & 0.16 & - & - & - \\
        \textbf{ALBETO} & - & - & - & - & - & - & 0.62 & - & - & - & - & - & - & - \\
        \textbf{AmRoBERTa} & - & 0.72 & - & - & - & - & - & - & - & - & - & - & - & - \\
        \textbf{ARBERT} & - & - & 0.56 & - & - & - & - & - & - & - & - & - & - & - \\
        \textbf{\texttt{arb} BERT} & - & - & 0.31 & - & - & - & - & - & - & - & - & - & - & - \\
        \textbf{BETO} & - & - & - & - & - & - & 0.68 & - & - & - & - & - & - & - \\

   \textbf{DziriBERT} & - & - & - & 0.43 & - & - & - & - & - & - & - & - &- & \\
     
           \textbf{Indic-BERT} & - & - & - & - & - & - & - & - &0.40 & - & -& 0.46 &-0.16  & 0.41\\
  
       \textbf{MARBERT} & - & - & 0.29 & - & - & - & - & - & - & - & - & - & - & - \\

  
        \textbf{RoBERTa-BNE} & - & - & - & - & - & - & 0.66 & - & - & - & - & - & - & - \\
        \textbf{HauRoBERTa} & - & - & - & - & - & - & - & 0.12 & - & - & - & - & - & - \\
        \midrule
        \textbf{} & \multicolumn{14}{c}{\textbf{Supervised}}  \\
        \midrule
         \textbf{LaBSE}& - & 0.85 & - & 0.60  & 0.77 & 0.83 & 0.70 & 0.69 & -  & - & 0.72 & 0.88 & - & 0.82 \\

        \midrule
        \textbf{} & \multicolumn{14}{c}{ \textbf{Crosslingual}} \\
        \midrule
        \textbf{LaBSE} & 0.79 & 0.84 & 0.61 & 0.46 & 0.40
 & 0.80 & 0.62 & 0.62
 & 0.76 & 0.47 & 0.57 & 0.84 & -0.05 & 0.82 \\
        \bottomrule[1.2pt]
    \end{tabular}
    \caption{Spearman correlation scores for different fine-tuned models in the three settings that we describe (supervised, unsupervised, and crosslingual) in addition to a simple lexical overlap baseline (Overlap).} 
    \label{tab:encoder-based-models}
%    }
\end{table*}
